Context-aware LLM-based Safe Control Against Latent Risks

Autonomous control systems face significant challenges in performing complex tasks in the presence of latent risks. To address this, we propose an integrated framework that combines Large Language Models (LLMs), numerical optimization, and optimization-based control to facilitate efficient subtask learning while ensuring safety against latent risks. The framework decomposes complex tasks into a sequence of context-aware subtasks that account for latent risks. These subtasks and their parameters are then refined through a multi-time-scale process: high-layer multi-turn in-context learning, mid-layer LLM Chain-of-Thought reasoning and numerical optimization, and low-layer model predictive control. The framework iteratively improves decisions by leveraging qualitative feedback and optimized trajectory data from lower-layer optimization processes and a physics simulator. We validate the proposed framework through simulated case studies involving robot arm and autonomous vehicle scenarios. The experiments demonstrate that the proposed framework can mediate actions based on the context and latent risks and learn complex behaviors efficiently.

==> algorithms/alg1_journal.tex <==
% version 3/28
% \begin{minipage}{\linewidth}
% \vspace{20.5cm}
% \enlargethispage{1\baselineskip}
% \vspace*{100em}
% \vspace{-30pt} 
\begin{algorithm}[!ht]
  \caption{Proposed framework (offline)}\label{alg:proposed_framework}
  \begin{algorithmic}[1]
    \Require $l$: task instructions, $I$: environment video clips, $x(0)$: initial state, $\mathcal{R}(x_{0:T},u_{0:T})$: evaluation metric, $\mathcal{B}_{\mathtt{s}}$: sequence of pairs of task and desirable subtask decomposition

    \Ensure $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted subtask sequence and optimized parameters, $\mathcal{B}_{\mathtt{s}}$: added sequence of pairs of task and desirable subtask decomposition
    
    \State \textbf{Initialize} $\mathcal{P}_{\mathtt{correction}},\mathcal{P}_{\mathtt{\mathtt{coder}}},\mathcal{B}_{\mathtt{f}}\gets \emptyset
    \Statex \Comment{prompts and memory buffers }
    \State \textbf{Initialize}  $\mathtt{LLM_{\mathtt{correction}}}(\mathcal{P}_{\mathtt{correction}}), \mathtt{LLM_{\mathtt{coder}}}(\mathcal{P}_{\mathtt{coder}})$
    \Statex \Comment{initialize LLMs with prompts}
    \State $t \gets 0,\ \epsilon \gets 10^{-3}$  \Comment{task clock, convergence threshold}
% \Comment{start the process}
    % \State $t \gets 0,\ \epsilon \gets 10e^{-3},\ \tau \gets 0\;$ \Comment{start the process}
    
    \State $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets$ Algorithm \ref{alg:context-resoning}$(l, I)$ 
    % \State $i \gets 1$ \Comment{start from the first subtask}

    % \Repeat $N_{\text{total}}$ \text{times}
    % \For {$\tau$ in $\{1,2,\cdots,N_{\text{total}}\}$}
    \While {$\mathtt{True}$}
    \State $x_{0:T}, u_{0:T}, \boldsymbol{D}, \xi $
    \Statex $\qquad\qquad \gets\text{Algorithm~\ref{alg:mpc}}(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}},x(t))$
    \Statex \Comment{run MPC for all the subtasks}
    % \State $D^{[i]}\gets \text{MPC sequence}\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$
    \If{$\boldsymbol{D}$ is $\mathtt{False}$}
    \State $\infty \gets \mathcal{R}(x_{0:T},u_{0:T})$ \Comment{task failed}
    \State $\mathcal{F}\gets \mathtt{FeedbackTemplate}(x_{0:T}, u_{0:T})$
    % \State $\mathcal{B}_{\mathtt{correction}}\gets \text{CONCAT}(\mathcal{B}_{\mathtt{correction}}, \mathcal{F})$ 
    % \Statex \Comment{append new correction $c$ to the correction buffer}
    \State $c\gets \mathtt{LLM_{correction}}(\mathcal{F})$
    \State $\mathcal{B}_{\mathtt{f}}\gets \text{CONCAT}(\{\mathcal{F}, c, \{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}\},\mathcal{B}_{\mathtt{f}})$
    \Statex \Comment{$\mathcal{F}$ is optional}
    % \State $\mathcal{B}_{\mathtt{coder}}\gets \text{CONCAT}(\mathcal{B}_{\mathtt{coder}}, c,\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i\in\mathcal{I}}, \mathcal{F})$ 
    % \Statex \Comment{append new correction $c$ to the correction buffer}
    % \State $\mathcal{B} \gets \text{CONCAT}(\mathcal{B}, c, \mathcal{F})$ 
    % \Statex \Comment{expand the memory buffer for the new failure case}
    % \State $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}-\xi}\gets \mathtt{LLM_{coder}}(c)$
    \State $\{R^{[j]},\boldsymbol{\Phi}^{[j]}, \param^{[j]}\}_{j\ge\xi}\gets \mathtt{LLM_{coder}}(\ell, \mathcal{B}_{\mathtt{f}}[1:\min(end,n_f)], \mathcal{B}_{\mathtt{s}}[1:\min(end,n_s)])$ 
    \Statex \Comment{update the parameters for the following subtasks, the total number of subtask $N = |\mathcal{I}|$ may change}
    \State $t \gets T-\omega^{[\xi]}$ \Comment{restart the failure subtask}
    \ElseIf{gradient $> L$} \Comment{the whole task succeeds}
    % \State Obtain $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
    %  \If{$\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}) \leq \epsilon$}  
    % \textbf{break} 
    % \EndIf \Comment{terminate the framework}
    % \State \textbf{Initialize} $N_{e},\,\eta_0,\,\gamma$ 
    % \Statex \Comment{$\#$ of iterations, initial learning rate, decay factor}
    % \For{$n$ in $\{1,2,\cdots,N_e\}$}
    %         \State $\eta \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}
    %         % \State Obtain $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ %\Comment{refer to Eq. (\ref{eq:gradient})}
    %         \State $\param \gets \param - \eta\cdot\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ 
    %         \State Recompute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
    %         % \State $n \gets n+1$
    % \EndFor
    
    
    \State $\{\param^{*[i]}\}_{i\in\mathcal{I}} \gets \mathtt{Optimize}_L(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
    \State $t \gets 0, \{\param\}_{i\in\mathcal{I}} \gets \{\param^{*[i]}\}_{i\in\mathcal{I}}$
    \Comment{termination condition $L$ of Optimize needs to match elseif condition}
    % \State $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}\gets$ 
    % \Statex \qquad\qquad Algorithm~\ref{alg:sgd} $(x_{0:T}, u_{0:T}, \{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}})$
    % \Statex \Comment{run SGD to optimize the subtasks}
    \Else
    \Comment{Optimized successful case}
    \State $\mathcal{F} \gets \mathtt{FeedbackTemplate}(x_{0:T}, u_{0:T})$
    \State $\mathcal{B}_{\mathtt{s}}\gets \text{CONCAT}(\{ \mathcal{F},\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{*[i]}\}_{i \in \mathcal{I}}\},\mathcal{B}_{\mathtt{s}})$
    
    \State \textbf{break} 
    \EndIf
    \If{$\mathtt{INTERRUPTION}$}  
    \textbf{break} 
    \Statex \Comment{termination from human or system-triggered event}
    \EndIf

    % \If{$\boldsymbol{D}$ is $\mathtt{True}$ and $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}) \leq \epsilon$}  
    % \State \textbf{break}
    % \EndIf
% \EndFor
\EndWhile


    % \While{$\boldsymbol{D}$ is $\mathtt{False}$}
    % \Statex \Comment{the whole task is not done}
    % \State $u_{t-{\omega^{[i]}}:t}, x_{t-{\omega^{[i]}}:t}, \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}},\boldsymbol{D}$ 
    % \Statex \qquad\qquad $ \gets$ Algorithm~\ref{alg:mpc}$(x(t), R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]},\boldsymbol{D})$ 
    % \Statex \Comment{refined subtask functions and parameters}
    % \State $i \gets i+1$
    % \EndWhile
    
    % \State $T \gets t$

    % \State $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}$ 
    % \Statex $\gets$ Algorithm~\ref{alg:llm_sgd_optimization} $(u_{0:T}, x_{0:T}, \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$  
    % \Statex\Comment{optimized subtask functions and their parameters}
    
  \end{algorithmic}
  
\end{algorithm}

% version before 3/28
% \begin{algorithm}[ht]
%   \caption{Offline procedure of the proposed framework}\label{alg:proposed_framework}
%   \begin{algorithmic}[1]
%     \Require $l$: task instruction, $I$: environment video clip, $x(0)$: initial state, $\boldsymbol{D}$: terminal statue for the whole task, $\mathtt{MAX\_subtasks}$: maximum number of subtasks

%     \Ensure $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted subtask sequence and optimized parameters
    
%     \State $t \gets 0$,\ $\boldsymbol{D}\gets \mathtt{False}$ \Comment{start the process}\;
%     \State $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets$ Algorithm \ref{alg:context-resoning}$(l, I)$ 
%     \State $i \gets 1$ \Comment{start from the first subtask}
%     \While{$\boldsymbol{D}$ is $\mathtt{False}$ and $i < \mathtt{MAX\_subtasks}$} 
%     \Statex \Comment{the whole task is not done, $\mathtt{MAX\_subtasks}$ helps to avoid infinite loop}
%     \State $u_{t-{\omega^{[i]}}:t}, x_{t-{\omega^{[i]}}:t}, \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}},\boldsymbol{D}$ 
%     \Statex \qquad\qquad $ \gets$ Algorithm~\ref{alg:mpc}$(x(t), R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]},\boldsymbol{D})$ 
%     \Statex \Comment{refined subtask functions and parameters}
%     \State $i \gets i+1$
%     \EndWhile
    
%     \State $T \gets t$

%     \State $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}$ 
%     \Statex $\gets$ Algorithm~\ref{alg:llm_sgd_optimization} $(u_{0:T}, x_{0:T}, \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$  
%     \Statex\Comment{optimized subtask functions and their parameters}
    
%   \end{algorithmic}
% \end{algorithm}
% \end{minipage}

==> algorithms/alg4_sgd.tex <==
% version 3/28
\begin{algorithm}[ht]
  \caption{Self-adaptive reasoning with SGD optimization (Section \ref{sec:llm_sgd})}\label{alg:sgd}
\begin{algorithmic}[1]
    \Require $u_{0:T}, x_{0:T}$: state and control histories, $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: rewards, subtask functions, and parameters
    \Ensure $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted rewards, subtask functions, and optimal parameter values

    \State \textbf{Initialize} $N_{e},\,\eta_0,\,\gamma$ 
    
    \Statex \Comment{$\#$ SGD iterations, initial learning rate, decay factor}

    \State $\epsilon \gets 10e^{-3}$\;

    \State Sample a mini-batch $\mathcal{B} \subseteq \{(u_t, x_t)\}_{t=0}^T$ \Comment{random subset of trajectory}
    \State Compute gradient $\nabla \mathcal{L}_{\mathcal{B}}(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ 


    \State $n \gets 1$

    \While{$\nabla \mathcal{L}_{\mathcal{B}}(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})>\epsilon$  and $n< N_e$}        
        \State $\eta \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}
        \State $\param \gets \param - \eta\cdot\GradientLshort_{\mathcal{B}}(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ 
        \Statex \Comment{update new parameters}
        
        \State Resample $\mathcal{B} \subseteq \{(u_t, x_t)\}_{t=0}^T$ and recompute $\GradientLshort_{\mathcal{B}}(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
        \State $n \gets n+1$
    \EndWhile

\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[ht]
%   \caption{Self-adaptive reasoning with SGD optimization (Section~\ref{sec:llm_sgd})}
%   \label{alg:sgd}
%   \begin{algorithmic}[1]
%     \Require 
%         $u_{0:T}, x_{0:T}$: state and control histories \\
%         $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: initial rewards, subtask functions, and parameters
%     \Ensure 
%         $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: optimized rewards, subtask functions, and parameters

%     \State \textbf{Initialize} $N_e$ (max iterations), $\eta_0$ (initial learning rate), $\gamma$ (decay rate), $\epsilon$ (convergence threshold)
%     \State $n \gets 0$

%     \Repeat
%         \State $\eta \gets \eta_0 \cdot e^{-\gamma n}$ \Comment{Exponential learning rate decay}
%         \State Compute gradient: $\nabla \mathcal{L} \gets \GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
%         \State $\param^{[i]} \gets \param^{[i]} - \eta \cdot \nabla \mathcal{L}^{[i]} \quad \forall i \in \mathcal{I}$ \Comment{Gradient update}
%         \State $n \gets n + 1$
%     \Until{$\|\nabla \mathcal{L}\| < \epsilon$ or $n \geq N_e$}

%   \end{algorithmic}
% \end{algorithm}

% version before 3/28
% \begin{algorithm}[ht]
%   % \setcounter{AlgoLine}{0}
%   \caption{Self-adaptive reasoning with SGD optimization (Section \ref{sec:llm_sgd})}\label{alg:llm_sgd_optimization}
% \begin{algorithmic}[1]
%     \Require $u_{0:T}, x_{0:T}$: state and control histories, $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: rewards, subtask functions, and parameters
%     \Ensure $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted rewards, subtask functions, and optimal parameter values
%     \State \textbf{Initialize} $N_{e},\,\eta_0,\,\gamma$ 
%     \Statex \Comment{$\#$ SGD iterations, initial learning rate, decay factor}
%     \State \textbf{Initialize} $\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ 
%     \Statex \Comment{LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}

%     \State $\epsilon \gets 10e^{-3}$\;

%     \State Compute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$\;

%     \While{$\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}) > \epsilon$}        

%         % \quan{need to rerun MPC for all subtasks with the current $\param$ to update $x_{0:T}, u_{0:T}$, how to denote this process; run 3-8 in Algorithm 1?}

%         \State Update $x_{0:T}, u_{0:T}$ \Comment{run Algorithm \ref{alg:proposed_framework}, lines 3-8}
        
%         \State $\mathcal{F} \gets x_{0:T}, u_{0:T}$
%         \State $c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ 
%         \Statex \Comment{obtain adjustment command from feedback text $\mathcal{F}$}
%         \State $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}}(c)$ 
%         \Statex \Comment{update reward and constraint functions}
%         \State $n \gets 1$
%         \For{$n=1$ to $N_e$}
%             \State $\eta \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}
%             \State Obtain $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ %\Comment{refer to Eq. (\ref{eq:gradient})}
%             \State $\param \gets \param - \eta\cdot\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ 
%             \Statex \Comment{update new parameters}
%             % \State $n \gets n+1$
%         \EndFor

%         % \State $u_{0:T}, x_{0:T} \gets$ Algorithm \ref{alg:mpc}$(x(t), R^{[i]},\Phi^{[i]}, \param^{[i]})$ $\forall i\in\mathcal{I}=\{1, 2, \cdots, N\}$ \Comment{{recompute sequence of \hspace*{38.5em}actions and states}}
        
%         \State Recompute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
%     \EndWhile
    
%     % \Return $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$
% \end{algorithmic}
% \end{algorithm}


==> backup/ProposedFramework.tex <==
\begin{algorithm}[ht]
  \caption{Subtask generation and contextual reasoning (Section~\ref{sec:subtask})}\label{alg:context-resoning}
  \begin{algorithmic}[1]
    \Require $l$: task instruction, $I$: environment video clip
    \Ensure $\{\Subtask, \param^{[i]}\}_{i\in \mathcal{I}}$: subtask's reward, safety specification functions and corresponding parameters
    \State \textbf{Initialize} $\mathcal{P}_{\mathtt{coder}}$, $\mathcal{P}_{\mathtt{latentobject}}$, $\mathcal{P}_{\mathtt{riskhandling}}$ \Comment{prompts}
    \Statex \textbf{Initialize} $\mathtt{LLM_{coder}}(\mathcal{P}_{\mathtt{coder}}), \mathtt{LLM_{latentobject}}(\mathcal{P}_{\mathtt{latentobject}})$ 
    \Statex $\mathtt{LLM_{riskhandling}}(\mathcal{P}_{\mathtt{riskhandling}})$ \Comment{LLMs with prompts}
    
    \State $l_{I} \gets \mathtt{LLM_{vision}}(I)$ \Comment{describe the image in text}
    \State $o\gets \mathtt{LLM_{latentobject}}(l, l_{I})$ 
    \Statex \Comment{obtain probable (latent-) risk-critical objects}
    \State $s \gets \mathtt{LLM_{riskhandling}}(o)$ 
    \Statex \Comment{obtain a proposal to achieve safe action}
    \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}}(l, s)$ 
    \Statex \Comment{obtain subtask specifications}
  \end{algorithmic}
\end{algorithm}


==> backup/backup_algo.tex <==
% \begin{algorithm}[h]
% \caption{Proposed Framework}\label{alg:proposed_framework}
% \begin{algorithmic}[1]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \renewcommand{\algorithmicfunction}{\textbf{procedure}}
% \Require $\mathcal{T}$: task instruction, $\mathcal{P}_\mathtt{X}$: LLM prompts
% \Ensure $u$: safe control action

% \State Initialize: $N_{E}$ \Comment{$\#$ Episode}
% \State Initialize: $\mathtt{LLM_{X}(\mathcal{P}_{\mathtt{X}}})$ \Comment{Initialize LLMs with specific prompts}

% % \State Initialize: $\mathtt{LLM_{coder}}(\mathcal{P}_{\mathtt{coder}})$, $\mathtt{LLM_{latentobject}}(\mathcal{P}_{\mathtt{latentobject}})$, $\mathtt{LLM_{safetyhandling}}(\mathcal{P}_{\mathtt{safetyhandling}})$,
% % $\mathtt{LLM_{query}}(\mathcal{P}_{\mathtt{query}})$,


% \State $R,\,\,\phi^{\theta} \gets \mathtt{LLM_{coder}}(\mathcal{T})$ \Comment{obtain reward and safety constraint function parameterized on $\theta$ given the task specification}
% \State $x_{0} \gets x$ \Comment{initialize state}

% \For{$k\in\{0, 1, \cdots, N_{E}-1\}$}
%     \State $I_{k} \gets \text{read an image}$
%     \State $\mathcal{O} \gets \mathtt{LLM_{latentobject}}(\mathcal{T}, I_{k})$ \Comment{obtain the latent-risk object that LLM thinks is the most probable}
%     \State $\mathcal{S} \gets \mathtt{LLM_{safetyhandling}}(\mathcal{O})$ \Comment{obtain the text of solutions to guarantee the safety of latent object $\mathcal{O}$}
%     \State $\Tilde{\phi} \gets \mathtt{LLM_{coder}}(\mathcal{S})$ \Comment{obtain constraint on the latent-risk object}
%     \State $u = K(x_{k}, R,\, [\phi^{\theta},\,\Tilde{\phi}])$ \Comment{run optimization-based controller to get action $u_{k}$}
%     \State $x_{k+1} \gets x$ \Comment{update state, sensor input}
%     \State $\mathtt{success} \gets \mathtt{LLM_{query}}(\mathcal{F}(x_{k+1}))$ \Comment{query LLM to see if the task has been completed, given feedback text $\mathcal{F}(x_{k+1})$}

%     \If{not $\mathtt{success}$} 
%         \State $\theta \gets U(\mathcal{F}(x_{k}))$ \Comment{run LLM and SGD optimization to update the parameter $\theta$}
%     \EndIf
% \EndFor

% \Function{$K$}{$x$, $R$,\,$\phi$} \Comment{\textbf{optimization-based control (Section 4.2)}}
% \State Initialize: $T$ \Comment{time horizon}
% \State Initialize: $u=\{u_{0}, u_{1}, \cdots, u_{T}\}$ 
% \Comment{initial sequence of actions over the time horizon}
% \State $x_{0} \gets x$ \Comment{initialize state} 
% \State $Q(u) = \mathbb{E}[\sum_{T}R(x_{t})]\,\,\text{s.t.}\,\,x_{t+1} = P(x_{t}, u_{t}),\,\,t\in\{0, 1, \cdots, T-1\}$ \Comment{compute expected accumulated reward over the time horizon}
% \State $u^{*} = \arg\max_{u}Q(u)\,\,\text{s.t.}\,\,\mathbf{\phi} \geq 0$ \Comment{run optimization to find optimal sequence of actions}
% \State \Return $\mathbf{u}^{*}_{0}$
% \EndFunction

% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[t]
% \caption{LLM and SGD optimization}\label{alg:llm_sgd_optimization}
% \begin{algorithmic}[1]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \renewcommand{\algorithmicfunction}{\textbf{procedure}}
% \Function{$U$}{$\mathcal{F}$,\,$R$} \Comment{\textbf{LLM + SGD optimization (Section 4.3)}}
% \State $\mathcal{C} \gets \mathtt{LLM_{correction}}(\mathcal{F})$ 
% \Comment{obtain the correction command from LLM given the feedback text $\mathcal{F}$}
% \State $\phi^{\theta} \gets \mathtt{LLM_{coder}}(\mathcal{C})$ \Comment{command LLM to update the constraint function with new parameter}

% \State $\theta_{0} \gets \theta$ \Comment{initialize parameter seed generated by LLM}
% \State Initialize: $N_{S},\,\,\eta > 0$ \Comment{$\#$ SGD iterations, learning rate}
% \State $x_{0} \gets x$ \Comment{initialize state}
% \State $c_{0} \gets -R(x_{o})$ \Comment{get initial cost, negating the reward}

% \For{$k\in\{0, 1, \cdots, N_{S}-1\}$}
%     \State $u = K(x_{k}, R,\, \phi^{\theta_{k}})$ \Comment{run optimization-based control in simulation, given the constraint function with updated param $\theta_{k}$}
%     \State $x_{k+1} \gets P(x_{k}, u)$ \Comment{update state, given current state $x_{k}$ and action $u$}
%     \State $L_{k+1} \gets -R(x_{k+1})$ \Comment{get the cost $r$ from the current state, negating the reward}
%     \State $\nabla{L} \gets L_{k+1} - L_{k}$ \Comment{compute the cost gradient}
%     \State $\theta_{k+1} = \theta_{k} - \eta\nabla{L}$ \Comment{Update the new parameter}
% \EndFor
% \State \Return $\theta_{N_{S}}$
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

==> backup/redesigned_algo.tex <==
\begin{algorithm}[ht]
  \caption{Overall procedure of the technique}\label{alg:proposed_framework}
  \begin{algorithmic}[1]
    \Require $l$: task instruction, $I$: environment video clip, $x(0)$: initial state, $\mathbf{D}$: terminal condition for the whole task

    \Ensure $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted subtask sequence and its optimized parameters
    
    \State $t \gets 0$ \Comment{start the process}\;
    % \State $D \gets$ False \;
    \State $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets$ Algorithm \ref{alg:context-resoning}$(l, I)$ \Comment{initial sequence of reward, constraint functions, and parameters}
    \State $i \gets 0$ \Comment{start from the first subtask}
    \While{$\mathbf{D}$ is $\mathtt{False}$} \Comment{if the task is not complete}
    \State $i \gets i+1$
    \State $u_{t-{\omega^{[i]}}:t}, x_{t-{\omega^{[i]}}:t}, \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets$ Algorithm~\ref{alg:mpc}$(R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]})$
    % \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \{R^{[i]*},\boldsymbol{\Phi}^{[i]*}, \param^{[i]*}\}_{i \in \mathcal{I}}$ 
    \Statex \Comment{update the subtask functions and parameters for the following subtasks}
    \EndWhile
    
    % \While{$i \in \mathcal{I}$} \Comment{execute one subtask}
    %     \State $u_{t-{\omega^{[i]*}}:t}, x_{t-{\omega^{[i]*}}:t}, \{R^{[i]*},\boldsymbol{\Phi}^{[i]*}, \param^{[i]*}\}_{i \in \mathcal{I}} \gets$ Algorithm~\ref{alg:mpc}$(R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]})$
    %     \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \{R^{[i]*},\boldsymbol{\Phi}^{[i]*}, \param^{[i]*}\}_{i \in \mathcal{I}}$ 
    %     \Statex \Comment{update the subtask functions and parameters for the following subtasks}
    % \EndWhile
    \State $T \gets t$

    
    % \For{$i \in \mathcal{I}$}
    
        % \quan{since we already had a loop to execute each subtask in Alg. 3, do we need the loop here? So, the input and output of Alg. 3 should be this one?
        % }
        
        % \State $u_{0:T}, x_{0:T} \gets$ Algorithm \ref{alg:mpc}$(x(0), \{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
        
        % \State $u_{t:t+\tau}, x_{t:t+\tau} \gets$ Algorithm \ref{alg:mpc}$(x(t), \{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$

        % \State $t \gets t+\tau$ \Comment{generate control actions in $\tau$ time steps}
    % \EndFor

    \State $\{\Subtask, \param^{[i]}\}_{i \in \mathcal{I}} \gets$ Algorithm \ref{alg:llm_sgd_optimization}$(u_{0:T}, x_{0:T}, \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$  
    \Statex\Comment{update subtask functions and their parameters}
    
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
  \caption{Subtask generation and contextual reasoning (Section \ref{sec:subtask})}\label{alg:context-resoning}
  \begin{algorithmic}[1]
    \Require $l$: task instruction, $I$: environment video clip
    \Ensure $\{\Subtask, \param^{[i]}\}_{i\in \mathcal{I}}$: subtask's reward, safety specification functions and corresponding parameters
    \State \textbf{Initialize} $\mathcal{P}_{\mathtt{coder}}$, $\mathcal{P}_{\mathtt{latentobject}}$, $\mathcal{P}_{\mathtt{riskhandling}}$ \Comment{initialize prompts}
    \State \textbf{Initialize} $\mathtt{LLM_{coder}}(\mathcal{P}_{\mathtt{coder}})$ \Comment{initialize LLMs with prompts}
    \State \textbf{Initialize} $\mathtt{LLM_{latentobject}}(\mathcal{P}_{\mathtt{latentobject}}), \mathtt{LLM_{riskhandling}}(\mathcal{P}_{\mathtt{riskhandling}})$
    
    \State $l_{I} \gets \mathtt{LLM_{vision}}(I)$ \Comment{describe the image in natural language, $l_{I}\in\mathcal{T}$}
    \State $o\gets \mathtt{LLM_{latentobject}}(l, l_{I})$ \Comment{obtain probable (latent-) risk object that LLM thinks is probable}
    \State $s \gets \mathtt{LLM_{riskhandling}}(o)$ \Comment{obtain a proposal to achieve safe action}
    \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}}(l, s)$ \Comment{obtain subtask specifications}
  \end{algorithmic}
\end{algorithm}

%% old version of alg3
% \begin{algorithm}[ht]
%   \caption{Optimization-based control (Section \ref{sec:mpc})}\label{alg:mpc}
%   \begin{algorithmic}[1]
%     \Require $x(0)$: current state, $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: subtask functions and parameters 
%     \Statex \Comment{subtasks termination condition $\{D^{[i]}(\cdot)\}_{i \in \mathcal{I}}$ and execution time window $\{\omega^{[i]}\}_{i \in \mathcal{I}}$ are included in the $\{\param^{[i]}\}_{i \in \mathcal{I}}$}
%     \Ensure $u_{0:T}, x_{0:T}$: state and control histories of given subtasks 
%     % \quan{Output: $u_{0:\tau}, x_{0:\tau}$?}
    
%     % \State $\tau\gets0$
%     \State $t \gets 0$
%     % \quan{$T \gets 0$?}
    
%     % \quan{what if in the following we check the evaluation function $D$ at $x(\tau)$, that is $D^{[i]}[x(\tau)]$, since at the first iteration we may not have access to $x(\tau + 1)$}
    
%     \For{$i\in\mathcal{I}$}
%         % \State $t_{\text{subtask}i} \gets 0$
%         \State $t_{\text{MPC}} \gets 0$
%         \While{$t_{\text{MPC}} < \omega^{[i]}$ and $D^{[i]}(x(t)) = 0$}
%             \State $u(t) = \text{MPC}[\RewardS,\,\ConstraintS]$ \Comment{obtained $u(t_{\text{MPC}})$ using Equation \ref{eq:mpc}}
%             \State $x(t+1) = f[x(t )] + g[x(t), u(t)]$
%             \State $t_{\text{MPC}} \gets t_{\text{MPC}}+1$
%             \State $t \gets t+1$
%             % \State $t \gets t+1$
%             \If{$D^{[i]}(x(t) =  1$}
%                 \State $i \gets i+1$
%                 \State $t \gets T$
%             \EndIf            
%         \EndWhile
%         \If{$D^{[i]}(x(t)) = 0$}
%         \State $\mathcal{F} \gets x_{t:T}, u_{t:T}$
%         \State $\mathtt{LLM_{correction}}(\mathcal{F})\gets c$
%         \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}(c)}$ 
%         % \xiyu{need to find a way to denote the following subtasks}

%         % \quan{do we need reset $\tau$ here, $\tau\gets0$}
        
%         \EndIf
%     \EndFor    
%   \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[ht]
  \caption{Optimization-based control (Section \ref{sec:mpc})}\label{alg:mpc}
  \begin{algorithmic}[1]
    \Require $x(t)$: current state, $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: subtask functions and parameters 
    \Statex \Comment{subtasks termination condition $\{D^{[i]}(\cdot)\}_{i \in \mathcal{I}}$ and execution time window $\{\omega^{[i]}\}_{i \in \mathcal{I}}$ are included in the $\{\param^{[i]}\}_{i \in \mathcal{I}}$}
    \Ensure $u_{t-\omega^{[i]}:t}, x_{t-\omega^{[i]}:t}$: state and control histories of given subtasks within the adjusted window $\omega^{[i]}$, 
    \Statex  $\qquad\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted subtask functions and parameters
    \State $t_{\text{MPC}} \gets 0$ \Comment{set the MPC clock}
    \While{$D^{[i]}$ is $\mathtt{False}$ and $t_{\text{MPC}}\leq \omega^{[i]}$}  \Comment{while the subtask is not complete}
        %\If{$t_{\text{MPC}}\leq \omega^{[i]}$} \Comment{if within time window}
        \State $u(t) = \text{MPC}[\RewardS,\,\ConstraintS,x(t)]$ \Comment{obtained $u(t)$ using Equation \ref{eq:mpc}}
        \State $x(t+1) = f[x(t)] + g[x(t), u(t)]$ \Comment{obtain the next state}
        \State $t_{\text{MPC}} \gets t_{\text{MPC}}+1$ \Comment{update MPC clock}
        \State $t\gets t+1$ \Comment{update natural clock}
        %\Else \Comment{if out of time}
     \EndWhile
     \If{$D^{[i]}(t)$ is $\mathtt{False}$} \Comment{if the subtask is fail}
     \State $\mathcal{F} \gets x_{t-\omega^{[i]}:t}, u_{t-\omega^{[i]}:t}$ \Comment{generate feedback text $\mathcal{F} \in \mathcal{T}$}
        \State $c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ \Comment{obtain correction command}
        \State $\{R^{[j]},\boldsymbol{\Phi}^{[j]}, \param^{[j]}\}_{j \in \{i+1,i+2,\cdots, N\}} \gets \mathtt{LLM_{coder}}(c)$  
        \Statex\Comment{update functions parameters for the following subtasks with updated number of total task $N$}
     \EndIf
        
        % \State $t_{\text{MPC}} \gets 0$ \Comment{reset the MPC clock}
        %\EndIf
   
    \State $\omega^{[i]} \gets t_{\text{MPC}}$ \Comment{for successful subtask, update the time usage $\omega^{[i]}$}
  \end{algorithmic}
\end{algorithm}

%% alg3 with 1 step each time
% \begin{algorithm}[ht]
%   \caption{Optimization-based control (Section \ref{sec:mpc})}\label{alg:mpc}
%   \begin{algorithmic}[1]
%     \Require $x(t)$: current state, $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: subtask functions and parameters 
%     \Statex \Comment{subtasks termination condition $\{D^{[i]}(\cdot)\}_{i \in \mathcal{I}}$ and execution time window $\{\omega^{[i]}\}_{i \in \mathcal{I}}$ are included in the $\{\param^{[i]}\}_{i \in \mathcal{I}}$}
%     \Ensure $u_{t:t+\omega^{[i]*}}, x_{t:t+\omega^{[i]*}}$: state and control histories of the given subtask 
%     \If{$D^{[i]}(x(t)) = \mathtt{True}$} \Comment{if the subtask is complete}
%     \State $i \gets i+1$ \Comment{switch to the next subtask}
%     \Else \Comment{if the subtask is not complete}
%     \If{$t_{\text{MPC}}\leq \omega^{[i]}$} \Comment{if within the task time window $\omega^{[i]}$}
%     \State $u(t) = \text{MPC}[\RewardS,\,\ConstraintS]$ \Comment{obtained $u(t_{\text{MPC}})$ using Equation \ref{eq:mpc}}
%     \State $x(t+1) = f[x(t)] + g[x(t), u(t)]$ \Comment{get the next state}
%     \State $t_{\text{MPC}} \gets t_{\text{MPC}}+1$ \Comment{update MPC clock}
%     \State $t\gets t+1$ \Comment{update natural clock}
%     % \If{$D^{[i]}(x(t)) = \mathtt{True}$}
%     \State \textbf{break} \Comment{break to check if the subtask is complete}
%     \Else \Comment{run out of time with unfinished subtask}
%     \State $\mathcal{F} \gets x_{t-\omega^{[i]}:t}, u_{t-\omega^{[i]}:t}$ \Comment{generate feedback text $\mathcal{F} \in \mathcal{T}$}
%     \State $\mathtt{LLM_{correction}}(\mathcal{F})\gets c$ \Comment{obtain correction command}
%     \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}(c)}$  \Comment{update the set of reward, constraint functions and parameters}
%     \EndIf
%     \EndIf
%     % \If
%     % \State $\mathcal{F} \gets x_{t:T}, u_{t:T}$
%     %     \State $\mathtt{LLM_{correction}}(\mathcal{F})\gets c$
%     %     \State $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}(c)}$ 
%     % \State 
%     % \EndIf
    
%     % \State $t \gets 0$
%         % \State $t_{\text{subtask}i} \gets 0$
%         % \State $t_{\text{MPC}} \gets 0$
%         % \While{$t_{\text{MPC}} < \omega^{[i]}$ and $D^{[i]}(x(T)) = 0$}
%         %     \State $u(T ) = \text{MPC}[\RewardS,\,\ConstraintS]$ \Comment{obtained $u(t_{\text{MPC}})$ using Equation \ref{eq:mpc}}
%         %     \State $x(T +1) = f[x(T )] + g[x(T ), u(T )]$
%         %     \State $t_{\text{MPC}} \gets t_{\text{MPC}}+1$
%         %     \State $T \gets T+1$
%         %     \If{$D^{[i]}(x(T) =  1$}
%         %         \State $i \gets i+1$
%         %         \State $t \gets T$
%         %     \EndIf            
%         % \EndWhile
%   \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[ht]
  % \setcounter{AlgoLine}{0}
  \caption{Self-adaptive Reasoning with SGD Optimization (Section \ref{sec:llm_sgd})}\label{alg:llm_sgd_optimization}
\begin{algorithmic}[1]
    \Require $u_{0:T}, x_{0:T}$: state and control histories,
    \Statex $\qquad \{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: rewards, subtask functions, and parameters
    \Ensure $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted rewards, subtask functions, and optimal parameter values
    \State \textbf{Initialize} $N_{e},\,\eta_0,\,\gamma$ \Comment{$\#$ SGD iterations, initial learning rate, decay factor}
    \State \textbf{Initialize} $\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ \Comment{prompt LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}

    \State $\epsilon \gets 10e^{-3}$\;

    \State Compute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$\;

    \While{$\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}) > \epsilon$}        

        % \quan{need to rerun MPC for all subtasks with the current $\param$ to update $x_{0:T}, u_{0:T}$, how to denote this process; run 3-8 in Algorithm 1?}

        \State Update $x_{0:T}, u_{0:T}$ \Comment{run Algorithm \ref{alg:proposed_framework}, lines 3-8}
        
        \State $\mathcal{F} \gets x_{0:T}, u_{0:T}$
        \State $c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ \Comment{obtain adjustment command from feedback text $\mathcal{F}$, $c\in \mathcal{T}$}
        \State $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}}(c)$ \Comment{update reward and constraint functions}
        
        \For{$n\in\{1, 2, \cdots, N_e\}$}
            \State $\eta \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}
            \State Obtain $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ %\Comment{refer to Eq. (\ref{eq:gradient})}
            \State $\param \gets \param - \eta\cdot\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ \Comment{update new parameters}
        \EndFor

        % \State $u_{0:T}, x_{0:T} \gets$ Algorithm \ref{alg:mpc}$(x(t), R^{[i]},\Phi^{[i]}, \param^{[i]})$ $\forall i\in\mathcal{I}=\{1, 2, \cdots, N\}$ \Comment{{recompute sequence of \hspace*{38.5em}actions and states}}
        
        \State Recompute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
    \EndWhile
    
    \Return $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$
\end{algorithmic}
\end{algorithm}

==> backup/sgd.tex <==
\begin{algorithm}[ht]
  % \setcounter{AlgoLine}{0}
  \caption{Self-adaptive reasoning with SGD optimization (Section \ref{sec:llm_sgd})}\label{alg:llm_sgd_optimization}
\begin{algorithmic}[1]
    \Require $u_{0:T}, x_{0:T}$: state and control histories, $\{R^{[i]},\boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: rewards, subtask functions, and parameters
    \Ensure $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$: adjusted rewards, subtask functions, and optimal parameter values
    \State \textbf{Initialize} $N_{e},\,\eta_0,\,\gamma$ 
    \Statex \Comment{$\#$ SGD iterations, initial learning rate, decay factor}
    \State \textbf{Initialize} $\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ 
    \Statex \Comment{LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}

    \State $\epsilon \gets 10e^{-3}$\;

    \State Compute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$\;

    \While{$\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}) > \epsilon$}        

        % \quan{need to rerun MPC for all subtasks with the current $\param$ to update $x_{0:T}, u_{0:T}$, how to denote this process; run 3-8 in Algorithm 1?}

        \State Update $x_{0:T}, u_{0:T}$ \Comment{run Algorithm \ref{alg:proposed_framework}, lines 3-8}
        
        \State $\mathcal{F} \gets x_{0:T}, u_{0:T}$
        \State $c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ 
        \Statex \Comment{obtain adjustment command from feedback text $\mathcal{F}$}
        \State $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}} \gets \mathtt{LLM_{coder}}(c)$ 
        \Statex \Comment{update reward and constraint functions}
        \State $n \gets 1$
        \For{$n=1$ to $N_e$}
            \State $\eta \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}
            \State Obtain $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ %\Comment{refer to Eq. (\ref{eq:gradient})}
            \State $\param \gets \param - \eta\cdot\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$ 
            \Statex \Comment{update new parameters}
            % \State $n \gets n+1$
        \EndFor

        % \State $u_{0:T}, x_{0:T} \gets$ Algorithm \ref{alg:mpc}$(x(t), R^{[i]},\Phi^{[i]}, \param^{[i]})$ $\forall i\in\mathcal{I}=\{1, 2, \cdots, N\}$ \Comment{{recompute sequence of \hspace*{38.5em}actions and states}}
        
        \State Recompute $\GradientLshort(\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}})$
    \EndWhile
    
    % \Return $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}_{i \in \mathcal{I}}$
\end{algorithmic}
\end{algorithm}


% % \begin{algorithm}[ht]
% % \caption{Self-adaptive Reasoning with SGD Optimization}\label{alg:llm_sgd_optimization}
% % \kwFunction({$U$}{($x$)} \Comment{\textbf{LLM + SGD optimization (Section \ref{sec:llm_sgd})}}){

% % \kwInit{$N_{e},\,N_{s},\,\eta_0,\,\gamma$ \Comment{$\#$ SGD iterations, task execution time, initial learning rate, decay factor}}
% % \kwInit{$\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ \Comment{prompt LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}}
% % \kwInit{$u_0$ \Comment{initialize action seed}}
% % $x_0 \gets x$ \Comment{assign initial system state}
% % \textcolor{gray}{// Start LLM loop}

% % \For{$n\in\{k(N_{e}+1)+1\,|\,\forall k\geq0\}$}{
% %     $c \gets \mathtt{LLM_{correction}}(f)$ 
% %     \Comment{obtain adjustment command from feedback text $f\in, \mathcal{F},\,c\in, \mathcal{T}$}\;
% %     $\{R_{\paramr^{i}}^{i}(x_t)\}_n, \{\Phi_{\paramc^{i}}^{i}(x_t)\}_n \gets \mathtt{LLM_{coder}}(c)$ \Comment{update reward and constraint functions}\;
% %     $\param_n \gets [\{\paramr^{i}\}, \{\paramc^{i}\}]_n$ \Comment{update new parameters as a seed for the next SGD iterations}\;
% %     \textcolor{gray}{// Start SGD loop to optimize $\param_n$}\;
    
% %     \For{$m\in\{n, n+1, \cdots, (n+N_e)-1\}$}{
        
% %         Obtain $\mathcal{D}(x^m_{0:T_N}, u^m_{0:T_N}; \param_m)$ using (\ref{eq:gradient}) \Comment{compute gradient at $\param_{m}$}\;
% %         $\eta_{m} \gets \eta_{0}\cdot e^{-\gamma m}$ \Comment{update learning rate}\;
% %         Obtain $\param_{m+1}$ using (\ref{eq:up_param}) \Comment{update new parameters}\;
% %     }
% %     Obtain $\mathcal{D}(\cdot; \param_{n+N_e})$ using (\ref{eq:loss}) \Comment{recompute the cost at the end of SGD loop}
    
% %     \If{$\mathcal{D}(\cdot; \param_{n+N_e}) < \epsilon_{T}$}{
% %         \Return $\{R_{\paramr^{i}}^{i}(x_t)\}_{n+N_e}, \{\Phi_{\paramc^{i}}^{i}(x_t)\}_{n+N_e}$ \;
% %     }
% % }
% % }
% % \end{algorithm}

% % \begin{algorithm}[ht]
% %   \caption{Self-adaptive Reasoning with SGD Optimization}\label{alg:llm_sgd_optimization}
% %   \kwFunction ({$U$}{($x$)} \Comment{\textbf{LLM + SGD optimization (Section \ref{sec:llm_sgd})}}){{
% %     \kwInit{$N_{e},\,N_{s},\,\eta_0,\,\gamma$ \Comment{$\#$ SGD iterations, task execution time, initial learning rate, decay factor}}
% %     \kwInit{$\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ \Comment{prompt LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}}
% %     \kwInit{$u_0$ \Comment{initialize action seed}}
% %     $x_0 \gets x$ \Comment{assign initial system state}
    
% %     % \textcolor{gray}{// Start LLM loop}
    
% %     \For{$n\in\{k(N_{e}+1)+1\,|\,\forall k\geq0\}$}{
% %         $c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ 
% %         \Comment{obtain adjustment command from feedback text $\mathcal{F}$, $c\in \mathcal{T}$}\;
        
% %         $\{R^{i},\Phi^{i}\}_n,\, \param_n \gets \mathtt{LLM_{coder}}(c)$ \Comment{update reward and constraint functions}\;
        
% %         % $\param_n \gets [\{\paramr^{i}\}, \{\paramc^{i}\}]_n$ \Comment{update new parameters as a seed for the next SGD iterations}\;
        
% %         % \textcolor{gray}{// Start SGD loop to optimize $\param_n$}\;
        
% %         \For{$m\in\{n, n+1, \cdots, (n+N_e)-1\}$}{
% %             % Obtain $\mathcal{D}(x^m_{0:T_N}, u^m_{0:T_N}; \param_m)$ using (\ref{eq:gradient}) \Comment{compute gradient at $\param_{m}$}\;
            
% %             $\eta_{m} \gets \eta_{0}\cdot e^{-\gamma m}$ \Comment{update learning rate}\;
            
% %             Obtain $\GradientLshort(R, \Phi, \param_m)$\;
            
% %             $\param_{m+1} = \param_{m} - \eta_{m}\cdot\GradientLshort(R, \Phi, \param_m)$ \Comment{update new parameters}\;
% %         }
% %         Obtain $\GradientLshort(R, \Phi, \param_{n+N_e})$\;
        
% %         \If{$\GradientLshort(R, \Phi, \param_{n+N_e}) < \epsilon_{T}$}{
        
% %             \Return $\{R^{i},\Phi^{i}\}_{n},\,\param_{n+N_e}$ \;
% %         }
% %     }
% %   }
% %   }
% %   % \vspace{-0.1cm}
% % \end{algorithm}

% \begin{algorithm}[ht]
%   % \setcounter{AlgoLine}{0}
%   \caption{Optimization-based control (Section \ref{sec:mpc})}\label{alg:mpc}
%   \begin{algorithmic}[1]
%     \Require $x(t)$: current state, $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}$: subtask functions and parameters
%     \Ensure $u_{t:t+\tau}, x_{t:t+\tau}$: state and control histories of given subtasks
    
%     % \State $\epsilon_{R} \gets 10e^{-3}$
    
%     % \While{$\nabla R^i > \epsilon_{R}$}
%     %     \State $u(T_{i-1}) = \text{MPC}_{t_s}[\RewardS,\,\ConstraintS]$ \Comment{obtained using Eq. \ref{eq:mpc}}
%     %     \State $x(T_{i-1}+1) = f + g$ \Comment{state resulted from $u(T_{i-1})$}
%     %     \State $T_{i-1} \gets T_{i-1} + 1$
%     % \EndWhile

%     % \State $T_{i} \gets t_s$
%     \State $\tau\gets0$
%     \State $t_\text{MPC} \gets t$
%     \For{$i\in\mathcal{I}_{t}$}
%         \State $\tau\gets \tau+\omega^{[i]}$
%         % \State $t_{0} \gets t$ 
%         % \State $t_{\text{MPC}} \gets 0$ \Comment{reset the MPC clock}
%         \While{$t_{\text{MPC}}\leq t+\tau$}
%             \State $u(t_\text{MPC} ) = \text{MPC}[\RewardS,\,\ConstraintS]$ \Comment{obtained $u(t_{\text{MPC}})$ using Equation \ref{eq:mpc}}
%             \State $x(t_\text{MPC} +1) = f[x(t_\text{MPC} )] + g[x(t_\text{MPC} ), u(t_\text{MPC} )]$
%             \State $t_{\text{MPC}} \gets t_{\text{MPC}}+1$
%             % \State $t \gets t+1$
%         \EndWhile
%     \EndFor    
%     \Return $u_{t:t+\tau}, x_{t:t+\tau}$
%   \end{algorithmic}
% \end{algorithm}

% % \begin{algorithm}[ht]
% %   % \setcounter{AlgoLine}{0}
% %   \caption{Optimization-based control (Section \ref{sec:mpc})}\label{alg:mpc}
% %   \begin{algorithmic}[1]
% %     \Require $x(t)$: current state, $\{R^{[i]}, \boldsymbol{\Phi}^{[i]}, \param^{[i]}\}$: subtask functions and parameters
% %     \Ensure $u_{t:t+\tau}, x_{t:t+\tau}$: state and control histories of given subtasks
    
% %     \State $\tau\gets0$
% %     \State $t_{\text{MPC}}\gets t$ \Comment{initialize the MPC clock}
% %     \For{$i\in\mathcal{I}_{t}$}
% %         \State $\tau\gets \tau+\omega^{[i]}$
% %         % \State $t_{0} \gets t$ 
% %         % \State $t_{\text{MPC}} \gets 0$ \Comment{reset the MPC clock}
% %         \While{$t_{\text{MPC}}\leq t+\tau$}
% %             \State $u(t_{\text{MPC}}) = \text{MPC}[\RewardS,\,\ConstraintS]$ \Comment{obtained using Eq. \ref{eq:mpc}}
% %             \State $x(t_{\text{MPC}}+1) = f[x(t_{\text{MPC}})] + g[x(t_{\text{MPC}}), u(t_{\text{MPC}})]$
% %             \State $t_{\text{MPC}} \gets t_{\text{MPC}}+1$
% %             % \State $t \gets t+1$
% %         \EndWhile
% %         % \State $\tau\gets \tau+\omega^{[i]}$
% %     \EndFor    
% %     \Return $u_{t:t+\tau}, x_{t:t+\tau}$
% %   \end{algorithmic}
% % \end{algorithm}


% % \begin{algorithm}[ht]
% % \setcounter{AlgoLine}{0}
% % \caption{Optimization-based control (Section \ref{sec:mpc})}\label{alg:mpc}
% %     % \KwIn{$x(t_s)$: current state, $\{R^{i},\Phi^{i}\}$: subtask functions, $\param$: subtask parameters}
% %     % \KwOut{$u_{0:T_N}, x_{0:T_N}$: state and control histories}
% %     % \kwInit{$T_{0} = 0$, and $T_{i}, \forall i \in\mathcal{I}$}
% %     % \nl\For{$i\in\mathcal{I}=\{1, 2, \cdots, N\}$}{
% %     %     \nl\For{${t_s}\in[T_{i}, T_{i+1}]$}{
% %     %         \nl$u(t_s) = \text{MPC}_{t_s}[\RewardS,\,\ConstraintS]$ \Comment{obtained using Eq. \ref{eq:mpc}}\;
% %     %         % $u_{T_{i-1}:T_i} = \{\text{MPC}_{t_s}[\cdot],\,\forall t_s\in [T_{i-1}, T_{i}]\}$ \Comment{control sequence of subtask $i$ (\ref{eq:mpc-subtask})}\;
            
% %     %         \nl$x(t_s+1) = f + g\cdot u(t_s)$ \Comment{state resulted from $u(t_s)$}\;
% %     %     }   
% %     % }
% %     % \nl\Return $u_{0:T_N}, x_{0:T_N}$ \Comment{$u_{0:T_N} = \{u(0), \cdots u(T_N)\}$, $x_{0:T_N} = \{x(0), \cdots x(T_N)\}$}\;

% %     \KwIn{$x(t_{s})$: current state, $R^{i},\Phi^{i},\param^{i}$: subtask functions and parameters}
% %     \KwOut{$u_{T_{i-1}:T_{i}}, x_{T_{i-1}:T_{i}}$: state and control histories of subtask $i$}
    
% %     \nl$\epsilon_{R} \gets 10e^{-3}$
        
% %     % \nl\For{${t_s}\in[T_{i-1}, T_{i}]$}{
% %     %     \nl$u(t_s) = \text{MPC}_{t_s}[\RewardS,\,\ConstraintS]$ \Comment{obtained using Eq. \ref{eq:mpc}}\;
% %     %     % $u_{T_{i-1}:T_i} = \{\text{MPC}_{t_s}[\cdot],\,\forall t_s\in [T_{i-1}, T_{i}]\}$ \Comment{control sequence of subtask $i$ (\ref{eq:mpc-subtask})}\;
        
% %     %     \nl$x(t_s) = f + g\cdot u(t_s)$ \Comment{state resulted from $u(t_s)$}\;
% %     % }   

% %     \nl\While{$\nabla R^i > \epsilon_{R}$}{
% %         \nl$u(t_s) = \text{MPC}_{t_s}[\RewardS,\,\ConstraintS]$ \Comment{obtained using Eq. \ref{eq:mpc}}\;
% %         % $u_{T_{i-1}:T_i} = \{\text{MPC}_{t_s}[\cdot],\,\forall t_s\in [T_{i-1}, T_{i}]\}$ \Comment{control sequence of subtask $i$ (\ref{eq:mpc-subtask})}\;
        
% %         \nl$x(t_s+1) = f + g\cdot u(t_s)$ \Comment{state resulted from $u(t_s)$}\;

% %         \nl$t_s \gets t_s + 1$
% %     }
% %     \nl$T_{i} \gets t_s$

% %     \nl\Return $u_{T_{i-1}:T_{i}}, x_{T_{i-1}:T_{i}}$ \;
    

% % \end{algorithm}


% \begin{algorithm}[ht]
%   % \setcounter{AlgoLine}{0}
%   \caption{Self-adaptive Reasoning with SGD Optimization (Section \ref{sec:llm_sgd})}\label{alg:llm_sgd_optimization}
% \begin{algorithmic}[1]
%     \Require $u_{0:T}, x_{0:T}$: state and control histories
%     \Ensure $\{\Subtask\}$: adjusted subtask functions, $\param$: optimal parameter values
%     \State \textbf{Initialize} $N_{e},\,\eta_0,\,\gamma$ \Comment{$\#$ SGD iterations, initial learning rate, decay factor}
%     \State \textbf{Initialize} $\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ \Comment{prompt LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}

%     \State $\epsilon \gets 10e^{-3}$\;

%     \State Compute $\GradientLshort(R, \boldsymbol{\Phi}, \param)$ with $x_{0:T}, u_{0:T}$\;

%     \While{$\GradientLshort(R, \boldsymbol{\Phi}, \param) > \epsilon$}
%         \State $\mathcal{F} \gets x_{0:T}, u_{0:T}$
%         \State $c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ \Comment{obtain adjustment command from feedback text $\mathcal{F}$, $c\in \mathcal{T}$}
%         \State $\{\Subtask\},\, \param \gets \mathtt{LLM_{coder}}(c)$ \Comment{update reward and constraint functions}
        
%         \For{$n\in\{1, 2, \cdots, N_e\}$}
%             \State Obtain $\GradientLshort(R, \boldsymbol{\Phi}, \param)$
%             \State $\eta \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}
%             \State $\param \gets \param - \eta\cdot\GradientLshort(R, \boldsymbol{\Phi}, \param)$ \Comment{update new parameters}
%         \EndFor

%         % \State $u_{0:T}, x_{0:T} \gets$ Algorithm \ref{alg:mpc}$(x(t), R^{[i]},\Phi^{[i]}, \param^{[i]})$ $\forall i\in\mathcal{I}=\{1, 2, \cdots, N\}$ \Comment{{recompute sequence of \hspace*{38.5em}actions and states}}
        
%         \State Recompute $\GradientLshort(R, \boldsymbol{\Phi}, \param)$ with the updated $u_{0:T}, x_{0:T}$
%     \EndWhile
    
%     \Return $\{\Subtask\},\,\param$
% \end{algorithmic}
% \end{algorithm}

% % \begin{algorithm}[ht]
% % \setcounter{AlgoLine}{0}
% %   \caption{Self-adaptive Reasoning with SGD Optimization (Section \ref{sec:llm_sgd})}\label{alg:llm_sgd_optimization}

% %     % \KwIn{$\{R^{i},\Phi^{i}\}_{0}$: initial subtask functions, $\param_{0}$: initial parameter values}
% %     \KwIn{$u_{0:T_{N}}, x_{0:T_{N}}$: state and control histories}
% %     \KwOut{$\{R^{i},\Phi^{i}\}$: adjusted subtask functions, $\param$: optimal parameter values}
% %     \kwInit{$N_{e},\,\eta_0,\,\gamma$ \Comment{$\#$ SGD iterations, initial learning rate, decay factor}}
% %     \kwInit{$\mathtt{LLM_{correction}}(\mathcal{P}_{\mathtt{correction}})$ \Comment{prompt LLM with $\mathcal{P}_{\mathtt{correction}}$ prompt text}}

% %     % \kwInit{$\{R^{i},\Phi^{i}\}\gets\{R^{i},\Phi^{i}\}_{0},\, \param\gets\param_{0}$ \Comment{$\param = \{\param^i\}$}}

% %     % \nl$u_{0:T_N}, x_{0:T_N} \gets$ Algorithm \ref{alg:mpc} $(\{R^{i},\Phi^{i},\param^i\})$

% %     \nl$\epsilon_{T} \gets 10e^{-3}$\;
    
% %     \nl Compute $\nabla\myL$ with $x_{0:T_N}, u_{0:T_N}$\;

% %     \nl\While{$\nabla\myL > \epsilon_{T}$}{
% %         \nl$\mathcal{F} \gets x_{0:T_N}, u_{0:T_N}$
    
% %         \nl$c \gets \mathtt{LLM_{correction}}(\mathcal{F})$ 
% %         \Comment{obtain adjustment command from feedback text $\mathcal{F}$, $c\in \mathcal{T}$}\;
        
% %         \nl$\{R^{i},\Phi^{i}\},\, \param \gets \mathtt{LLM_{coder}}(c)$ \Comment{update reward and constraint functions}\;
    
% %         \nl\For{$n\in\{1, 2, \cdots, N_e\}$}{
    
% %             \nl$\eta_{n} \gets \eta_{0}\cdot e^{-\gamma n}$ \Comment{update learning rate}\;
            
% %             \nl Obtain $\GradientLshort(R, \Phi, \param)$\;
            
% %             \nl$\param \gets \param - \eta_{n}\cdot\GradientLshort(R, \Phi, \param)$ \Comment{update new parameters}\;
% %         }

% %         \nl$u_{T_{i-1}:T_{i}}, x_{T_{i-1}:T_{i}} \gets$ Algorithm \ref{alg:mpc}$(x(t_s), R^{i},\Phi^{i}, \param^i)$ $\forall i\in\mathcal{I}=\{1, 2, \cdots, N\}$ \Comment{recompute sequence of actions and states}\;
        
% %         \nl Recompute $\nabla\myL$ with the updated $u_{0:T_N}, x_{0:T_N}$\;
% %     }
    
% %     \nl\Return $\{R^{i},\Phi^{i}\},\,\param$ \;
    
% %   % \vspace{-0.1cm}
% % \end{algorithm}

